What can Large Language Models Capture about Code Functional Equivalence?

Code-LLMs, LLMs pre-trained on large code corpora, have shown great progress in learning rich representations of the structure and syntax of code, successfully using it to generate or classify code fragments. At the same time, understanding if they are able to do so because they capture code semantics, and how well, is still an open question. In this paper, we tackle this problem by introducing SeqCoBench, a benchmark for systematically assessing how Code-LLMs can capture code functional equivalence. SeqCoBench contains over 20 code transformations that either preserve or alter the semantics of Python programs. We conduct extensive evaluations in different settings, including zero-shot and parameter-efficient finetuning methods on state-of-the-art (Code)-LLMs to see if they can discern semantically equivalent or different pairs of programs in SeqCoBench. We find that the performance gap between these LLMs and classical match-based retrieval scores is minimal, with both approaches showing a concerning lack of depth in understanding code semantics.

==> figures/motivating_example.tex <==
\begin{figure*}[t]
\begin{center}
\begin{tcbraster}[raster columns=3, raster rows=1, raster column skip=2mm, raster width=\linewidth, raster equal height]
%\begin{figure*}[t]
\setminted{fontsize=\tiny,framesep=1mm}
% \usemintedstyle{vs}
\begin{tcolorbox}[enhanced,frame hidden,boxrule=1pt,coltitle=black,title=\textcolor{white}{\footnotesize{{Code Summarization}}},colback=floralwhite,borderline= {0.75pt}{0pt}{lightgray,dashed},left=.1em, right=.1em, top=.1em, bottom=.1em,
subtitle style={boxrule=0pt,colback=babyblue},attach boxed title to top center={yshift*=-3mm},boxed title style={},
center title]
\textbf{\footnotesize{Prompt:}} \footnotesize{Summarize the code as a docstring in a few lines}
\begin{minted}[autogobble,numberblanklines=false,breaklines,tabsize=2,breaksymbolleft=]{python}
    def any_int(x, y, z):
        if isinstance(x,int) and isinstance(y,int) and isinstance(z,int):
            if (x+y==z) or (x+z==y) or (y+z==x):
                return True
            return False
        return False
\end{minted}
\tcbsubtitle{\centering\footnotesize{Summarization by \textbf{\texttt{CL-Inst-7B}}}}
\begin{minted}[autogobble,numberblanklines=false,frame=lines,breaklines,tabsize=2,breaksymbolleft=]{python}
"""This function takes three arguments x, y, and z, and returns True if any two of them add up to the third, or if the sum of two and three is equal to the third. Otherwise, it returns False."""
\end{minted}
\centering\textcolor{bostonuniversityred}{\faTimesCircle}\textbf{\footnotesize{\textcolor{bostonuniversityred}{{ }Missed Data Type}}}\\(No mention of integer type)
\end{tcolorbox} 
\begin{tcolorbox}[minipage boxed title*=-2cm,enhanced,frame hidden,boxrule=1pt,coltitle=black,title=\textcolor{white}{\small{{Code Summarization modified}}},colback=floralwhite,borderline= {0.75pt}{0pt}{lightgray,dashed},left=.1em, right=.1em, top=.1em, bottom=.1em,subtitle style={boxrule=0pt,colback=babyblue},attach boxed title to top center={yshift*=-3mm},boxed title style={},
center title]
\textbf{\footnotesize{Prompt:}} \footnotesize{Summarize the code as a docstring in a few lines}
\begin{minted}[autogobble,numberblanklines=false,breaklines,tabsize=2,breaksymbolleft=]{python}
    def any_int(x, y, z):
        if isinstance(x,int) and isinstance(y,float) and isinstance(z,int):
            if (x+y==z) or (x+z==y) or (y+z==x):
                return True
            return False
        return False
\end{minted}
\tcbsubtitle{\centering\footnotesize{Summarization by \textbf{\texttt{CL-Inst-7B}}}}
\begin{minted}[autogobble,numberblanklines=false,frame=lines,breaklines,tabsize=2,breaksymbolleft=]{python}
"""This function takes three arguments `x`, `y`, and `z` and returns `True` if any two of them add up to the third one, and `False` otherwise. The function first checks if all three arguments are of type `int` using the `isinstance()` function. If the arguments are not all of type `int`, the function returns `False`. If the arguments are all of type `int`, the function checks if any two of them add up to the third one using the `+` operator..."""
\end{minted}
\centering\textcolor{bostonuniversityred}
{\faTimesCircle}\textbf{\footnotesize{\textcolor{bostonuniversityred}{{ }Wrong Data Type}}}\\(\texttt{float} type incorrectly considered as \texttt{int})
\end{tcolorbox}
\begin{tcolorbox}[enhanced,frame hidden,boxrule=1pt,coltitle=black,title=\textcolor{white}{\footnotesize{{Code Execution reasoning}}},colback=floralwhite,borderline= {0.75pt}{0pt}{lightgray,dashed},left=.1em, right=.1em, top=.1em, bottom=.1em,subtitle style={boxrule=0pt,colback=babyblue},attach boxed title to top center={yshift*=-3mm},boxed title style={},
center title]
\textbf{\footnotesize{Prompt:}} \footnotesize{Given the input=[3,2,2], what would be the output by the code below?}
\begin{minted}[autogobble,numberblanklines=false,breaklines,tabsize=2,breaksymbolleft=]{python}
    def any_int(x, y, z):
        if isinstance(x,int) and isinstance(y,int) and isinstance(z,int):
            if (x+y==z) or (x+z==y) or (y+z==x):
                return True
            return False
        return False
\end{minted}
\tcbsubtitle{\centering\footnotesize{Reasoning by \textbf{\texttt{CL-Inst-7B}}}}
\begin{minted}[autogobble,numberblanklines=false,frame=lines,breaklines,tabsize=2,breaksymbolleft=]{console}
The output of the code would be `True`, since the condition `x+y==z` is satisfied.
\end{minted}
\centering\textcolor{bostonuniversityred}{\faTimesCircle}\textbf{\footnotesize{\textcolor{bostonuniversityred}{{ }Wrong Data Value}}}\\(Actual output is \texttt{False} and explanation about reasoning is incorrect)
\end{tcolorbox}
\end{tcbraster}
\end{center}
\caption{
\AV{I'd put here some examples of failures out of our benchmark, for some (if not all) transformations.}
\textbf{CodeLLMs do not fully capture the underlying semantics as they struggle to identify the exact data type, identify the wrong type altogether, and fail to predict the correct output upon execution.} An example based on \texttt{HumanEval/92} to show shallow code understanding abilities of CodeLLMs. \texttt{CL-Inst-7B:} Code-Llama-Instruct-7B.}
\vspace*{-1em}
\label{fig:motivating-example}
\end{figure*}

